Consensus and Subjectivity of Skin Tone Annotation for ML Fairness

Understanding different human attributes and how they affect model behavior may become a standard need for all model creation and usage, from traditional computer vision tasks to the newest multimodal generative AI systems. In computer vision specifically, we have relied on datasets augmented with perceived attribute signals (e.g., gender presentation, skin tone, and age) and benchmarks enabled by these datasets. Typically labels for these tasks come from human annotators. However, annotating attribute signals, especially skin tone, is a difficult and subjective task. Perceived skin tone is affected by technical factors, like lighting conditions, and social factors that shape an annotator's lived experience. This paper examines the subjectivity of skin tone annotation through a series of annotation experiments using the Monk Skin Tone (MST) scale, a small pool of professional photographers, and a much larger pool of trained crowdsourced annotators. Along with this study we release the Monk Skin Tone Examples (MST-E) dataset, containing 1515 images and 31 videos spread across the full MST scale. MST-E is designed to help train human annotators to annotate MST effectively. Our study shows that annotators can reliably annotate skin tone in a way that aligns with an expert in the MST scale, even under challenging environmental conditions. We also find evidence that annotators from different geographic regions rely on different mental models of MST categories resulting in annotations that systematically vary across regions. Given this, we advise practitioners to use a diverse set of annotators and a higher replication count for each image when annotating skin tone for fairness research.

==> old_results.tex <==










    























==> paper_checklist.tex <==
\begin{enumerate}
    \item For all authors
    \begin{enumerate}
        \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
        \begin{itemize}
            \item Yes.
        \end{itemize}
        \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
        \begin{itemize}
            \item Yes.
        \end{itemize}
        \item Did you discuss any potential negative societal impacts of your work?
        \begin{itemize}
            \item Yes. See "Limitations and Ethical Considerations" in Section~\ref{sec:discussion}.
        \end{itemize}
        \item Did you describe the limitations of your work?
        \begin{itemize}
            \item Yes. See "Limitations and Ethical Considerations" in Section~\ref{sec:discussion}.
        \end{itemize}
    \end{enumerate}
    \item If you are including theoretical results
    \begin{itemize}
        \item We do not include theoretical results.
    \end{itemize}
    \item If you ran experiments
    \begin{enumerate}
        \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
        \begin{itemize}
            \item Yes, annotations can be found at {\color{blue}{\url{https://storage.googleapis.com/mste/mste_annotations.csv}}}. See Appendix~\ref{app:datacard} for more details.
        \end{itemize}
        \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
        \begin{itemize}
            \item N/A. We did not train a model.
        \end{itemize}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        \begin{itemize}
            \item N/A. Plots show counts or statistical scores. All $p$ values are included in the text.
        \end{itemize}
        \item Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
        \begin{itemize}
            \item N/A. We did not train a model.
        \end{itemize}
    \end{enumerate}
    \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets
    \begin{enumerate}
        \item If your work uses existing assets, did you cite the creators?
        \begin{itemize}
            \item We extend and replicate the findings shown on the MST-E dataset to a large-scale image dataset using a subsample of Open Images. We cite the authors of the Open Images dataset~\cite{Kuznetsova20:Open}.
        \end{itemize}
        \item Did you mention the license of the assets?
        \begin{itemize}
            \item Yes, \link{https://creativecommons.org/licenses/by/4.0/}{CC BY}.
        \end{itemize}
        \item Did you include any new assets either in the supplemental material or as a URL?
        \begin{itemize}
            \item Yes, the dataset can be found at \link{https:\\skintone.google/mste-dataset}{skintone.google/mste-dataset}
        \end{itemize}
        \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
        \begin{itemize}
            \item Yes. The subjects in the MST-E dataset consented for their images to be used for research or human annotator training.
        \end{itemize}
        \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
        \begin{itemize}
            \item Yes, we are only releasing the skin tone annotations of the subjects in the MST-E dataset. All other sensitive attributes (age, gender identity) were not gathered from the subjects.
        \end{itemize}
    \end{enumerate}
    \item If you used crowdsourcing or conducted research with human subjects
    \begin{enumerate}
        \item Did you include the full text of instructions given to participants and screenshots, if applicable?
        \begin{itemize}
            \item Yes. See Appendix~\ref{app:task}.
        \end{itemize}
        \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
        \begin{itemize}
            \item Annotation experiments were conducted under the guidance of our institution's ethics body. No PII besides country of residence was collected from annotators. The images shown did not include offensive content.
        \end{itemize}
        \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
        \begin{itemize}
            \item Yes. See appendix~\ref{app:comp}.
        \end{itemize}
    \end{enumerate}
\end{enumerate}

==> paper_checklist_new.tex <==



\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See ``Limitations and Ethical Considerations'' in Section~\ref{sec:discussion}} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See ``Limitations and Ethical Considerations'' in Section~\ref{sec:discussion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Annotations can be found at {\color{blue}{\url{https://storage.googleapis.com/mste/mste_annotations.csv}}}. See Appendix~\ref{app:datacard} for more details.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{We did not train a model.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{Plots show counts or statistical scores. All $p$ values are included in the text.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{We did not train a model.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We extend and replicate the findings shown on the MST-E dataset to a large-scale image dataset using a subsample of Open Images. We cite the authors of the Open Images dataset~\cite{Kuznetsova20:Open}.}
  \item Did you mention the license of the assets?
    \answerYes{\link{https://creativecommons.org/licenses/by/4.0/}{CC BY}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The dataset can be found at \link{https:\\skintone.google/mste-dataset}{skintone.google/mste-dataset}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{The subjects in the MST-E dataset consented for their images to be used for research or human annotator training.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We are only releasing the skin tone annotations of the subjects in the MST-E dataset. All other sensitive attributes (age, gender identity) were not gathered from the subjects.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See Appendix~\ref{app:task}.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{Annotation experiments were conducted under the guidance of our institution's ethics body. No PII besides country of residence was collected from annotators. The images shown did not include offensive content.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See Appendix~\ref{app:comp}}
\end{enumerate}

\end{enumerate}
